Image-Binary Automata

We introduce a certain restriction of weighted automata over the rationals, called image-binary automata. We show that such automata accept the regular languages, can be exponentially more succinct than corresponding NFAs, and allow for polynomial complementation, union, and intersection. This compares favourably with unambiguous automata whose complementation requires a superpolynomial state blowup. We also study an infinite-word version, image-binary B\"uchi automata. We show that such automata are amenable to probabilistic model checking, similarly to unambiguous B\"uchi automata. We provide algorithms to translate $k$-ambiguous B\"uchi automata to image-binary B\"uchi automata, leading to model-checking algorithms with optimal computational complexity.

==> macros.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%%     Macros, newcommands and defs
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\barQ}{\overline{Q}}
\newcommand{\barn}{\overline{n}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%%    Ende
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\def\Ende{\hfill {\tiny $\blacksquare$}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%
%%%%     eqdef and angled brackets
%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\eqdef{\stackrel{\text{def}}{=}}

\def\<{\langle}
\def\>{\rangle}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%%    number sets
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\Nat{\mathbb{N}}
\def\Integer{\mathbb{Z}}
\def\Real{\mathbb{R}}
\def\Rational{\mathbb{Q}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%%    mathcal letters
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cI{\mathcal{I}}
\def\cJ{\mathcal{J}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cQ{\mathcal{Q}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cU{\mathcal{U}}
\def\cV{\mathcal{V}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%%     Fraktur font letters
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\fA{\mathfrak{A}}
\def\fB{\mathfrak{B}}
\def\fC{\mathfrak{C}}
\def\fD{\mathfrak{D}}
\def\fE{\mathfrak{E}}
\def\fF{\mathfrak{F}}
\def\fG{\mathfrak{G}}
\def\fH{\mathfrak{H}}
\def\fI{\mathfrak{I}}
\def\fJ{\mathfrak{J}}
\def\fK{\mathfrak{K}}
\def\fL{\mathfrak{L}}
\def\fM{\mathfrak{M}}
\def\fN{\mathfrak{N}}
\def\fO{\mathfrak{O}}
\def\fP{\mathfrak{P}}
\def\fQ{\mathfrak{Q}}
\def\fR{\mathfrak{R}}
\def\fS{\mathfrak{S}}
\def\fT{\mathfrak{T}}
\def\fU{\mathfrak{U}}
\def\fV{\mathfrak{V}}
\def\fW{\mathfrak{W}}
\def\fX{\mathfrak{X}}
\def\fY{\mathfrak{Y}}
\def\fZ{\mathfrak{Z}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%%     complexity classes
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\PTIME}{\mathrm{P}}
\newcommand{\NP}{\mathrm{NP}}
\newcommand{\coNP}{\mathrm{coNP}}
\newcommand{\PSPACE}{\mathrm{PSPACE}}
\newcommand{\EXPTIME}{\mathrm{EXPTIME}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%%    assorted macros
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\A}{\mathcal{A}}
\newcommand{\AF}{\overrightarrow{\mathcal{A}}}
\newcommand{\Bh}{\widehat{B}}
\newcommand{\alphaF}{\overrightarrow{\alpha}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\C}{\mathcal{C}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\Fh}{\widehat{F}}
\newcommand{\kA}{\mathcal{A}_k}
\newcommand{\MF}{\overrightarrow{M}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\QF}{\overrightarrow{Q}}
\newcommand{\R}{\mathbb{R}}
\DeclareMathOperator{\rank}{rank}
\newcommand{\VV}{\mathsf{V}}
\newcommand{\Z}{\mathbb{Z}}

\DeclareMathOperator{\prob}{\mathit{Pr}}
\DeclareMathOperator{\expect}{\mathbb{E}}
\newcommand{\paths}{\mathit{Paths}}
\DeclareMathOperator{\kdis}{\mathnormal{k}-dis}
\newcommand{\pow}{\mathcal{P}}



\def\Pr{\mathrm{Pr}}

\def\Paths{\mathit{Paths}}
\def\Act{\mathit{Act}}
\def\AP{\mathit{AP}}
\def\Acc{\mathit{Acc}}
\def\accEC{\mathit{accEC}}
\def\trace{\mathit{trace}}
\def\lab{\mathit{lab}}
\def\Post{\mathrm{Post}}

\def\qinit{q_{\textit{\tiny init}}}
\def\qtrap{q_{\textit{\tiny trap}}}
\def\qfinal{q_{\textit{\tiny final}}}

\def\qfinal{\mathit{final}}

\def\QSCC{Q_{\mathit{SCC}}^{>0}}
\def\QBSCC{Q_{\mathit{BSCC}}}
\def\Qunknown{Q_{?}}

\newcommand{\scc}[1]{\cC_{#1}}

\def\trace{\mathit{trace}}
\def\accrun{\mathit{accrun}}
\def\Runs{\mathit{Runs}}
\def\Pref{\mathit{Pref}}

\newcommand{\SCC}[1]{\mathit{SCC}(#1)}

\def\Cyl{\mathit{Cyl}}

\def\first{\mathit{first}}
\def\last{\mathit{last}}

\def\infoften{\mathit{inf}}

\def\cLomega{\cL_{\omega}}
\def\cLfin{\cL_{\textit{\tiny fin}}}

\def\sched{\mathfrak{S}}


\newcommand{\move}[1]{\stackrel{#1}{\longrightarrow}}

\newcommand{\sroot}[1]{\mathit{root}(#1)}

\newcommand{\notapplicable}{}
\newcommand{\subpointone}{\,$<\!\psec{0.1}$}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\extended}[1]{\hat{#1}}
\newcommand{\detlim}[1]{#1_{\text{\tiny \rm detlim}}}
\newcommand{\Det}[1]{#1_{\text{\tiny \rm det}}}

\newcommand{\NFA}[1]{#1_{\text{\tiny \rm NFA}}^{\text{\tiny all}}}

% Monotone closure operator
\newcommand{\Mon}{\mathit{Mon}}
%\newcommand{\det}[1]{{\text{\rm det}(\#)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%
%%%%    LTL operators
%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\until}{\cU}
\newcommand{\finally}{\Diamond}
\newcommand{\globally}{\Box}
\newcommand{\neXt}{\bigcirc}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%
%%%%    Numprint
%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\psec}[1]{\nprounddigits{1}\npfourdigitnosep\numprint[s]{#1}}
\newcommand{\pnodes}[1]{\nprounddigits{0}\numprint{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%
%%%%    Tools
%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\prism}{\texttt{PRISM}}
\newcommand{\colt}{\texttt{COLT}}
\newcommand{\spot}{\texttt{SPOT}}
\newcommand{\ltltodstar}{\texttt{ltl2dstar}}
\newcommand{\ltltotgba}{\texttt{ltl2tgba}}
\newcommand{\rabinizer}{\texttt{Rabinizer}}
\newcommand{\tulip}{\texttt{Tulip}}
\newcommand{\iscasmc}{\texttt{IscasMC}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%
%%%%    Function and variable names
%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\CoPath}{\mathit{CoPath}}
\newcommand{\Co}{\mathit{Co}}
\newcommand{\Survives}{\mathit{Survives}}
\newcommand{\unvisited}{\mathit{worklist}}

%% removed for final version:

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%
%%%%    Personal TODO notes
%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\todowithauthor}[4]{\todo[linecolor=gray,backgroundcolor=#3, #1]{#2\hfill{\scriptsize{\em{#4}}}}}

%\colorlet{christelColor}{Apricot!30!white}
%\colorlet{joachimColor}{Cerulean!30!white}
\colorlet{davidColor}{YellowGreen!30!white}
%\colorlet{saschaColor}{Purple!30!white}
\colorlet{stefanColor}{Brown!30!white}
\colorlet{benColor}{Yellow!30!white}


%\newcommand{\todoChristel}[2][]{\todowithauthor{#1}{#2}{christelColor}{Christel}}
%\newcommand{\todoJoachim}[2][]{\todowithauthor{#1}{#2}{joachimColor}{Joachim}}
\newcommand{\todoDavid}[2][]{\todowithauthor{#1}{#2}{davidColor}{David}}
%\newcommand{\todoSascha}[2][]{\todowithauthor{#1}{#2}{saschaColor}{Sascha}}

\newcommand{\todoStefan}[2][]{\todowithauthor{#1}{#2}{stefanColor}{Stefan}}
\newcommand{\todoBen}[2][]{\todowithauthor{#1}{#2}{benColor}{Ben}}




%-- For Emacs, please don't remove:
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:



==> preamble.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%%     usepackages
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% removed for final version:
\usepackage[dvipsnames]{xcolor}
\usepackage[backgroundcolor=magenta!10!white]{todonotes}

\usepackage{microtype}
%\usepackage[utf8]{inputenc}

%\usepackage{gastex}
%\usepackage{amsmath,amsthm,amssymb,amsfonts}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{thm-restate}
\declaretheorem[name=Theorem,style=plain,sibling=theorem]{ourtheorem}
\declaretheorem[name=Corollary,sibling=theorem]{ourcorollary}
\declaretheorem[name=Lemma,Refname={Lemma,Lemmas},sibling=theorem]{ourlemma}
\declaretheorem[name=Proposition,Refname={Proposition,Propositions},sibling=theorem]{ourproposition}

\usepackage{graphicx}

%\usepackage{subfigure}

%\usepackage[T1]{fontenc}

\usepackage{ifthen}

\usepackage{numprint}
\npdecimalsign{.}
\npthousandsep{,}

\usepackage{hyperref}
%\usepackage{algorithm2e}
%\usepackage{cleveref}
\usepackage{tikz}
\usetikzlibrary{arrows,automata,positioning,calc,intersections}
\usepackage{xcolor}


%% Colors: for review/editing phase, REMOVED FOR CAMERA READY
%\definecolor{highlightForUs}{rgb}{0.0,0.7,0.0}  % <- green
%\definecolor{highlightForUs}{rgb}{0.0,0.0,0.0}  % <- black
%\definecolor{highlightForReviewers}{rgb}{1.0,0.0,0.0}
%\definecolor{highlightForReviewers}{rgb}{0.0,0.0,0.0}  % <- black


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%%     theorems and co
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% already defined by llncs style:
%
%\newtheorem{definition}{Definition}[section]
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}{Lemma}[section]
%\newtheorem{proposition}{Proposition}[section]
%\newtheorem{corollary}{Corollary}[section]
%\newtheorem{example}{Example}[section]
%\newtheorem{remark}{Remark}[section]
%\newtheorem{notation}[definition]{Notation}
%\newtheorem{fact}[definition]{Fact}

% Add qed symbol to the end of proofs
%\usepackage{etoolbox}
%\AtEndEnvironment{proof}{\qed}




%-- For Emacs, please don't remove:
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

